Personalized Image Generation for Recommendations Beyond Catalogs

Personalization is central to human-AI interaction, yet current diffusion-based image generation systems remain largely insensitive to user diversity. Existing attempts to address this often rely on costly paired preference data or introduce latency through Large Language Models. In this work, we introduce REBECA (REcommendations BEyond CAtalogs), a lightweight and scalable framework for personalized image generation that learns directly from implicit feedback signals such as likes, ratings, and clicks. Instead of fine-tuning the underlying diffusion model, REBECA employs a two-stage process: training a conditional diffusion model to sample user- and rating-specific image embeddings, which are subsequently decoded into images using a pretrained diffusion backbone. This approach enables efficient, fine-tuning-free personalization across large user bases. We rigorously evaluate REBECA on real-world datasets, proposing a novel statistical personalization verifier and a permutation-based hypothesis test to assess preference alignment. Our results demonstrate that REBECA consistently produces high-fidelity images tailored to individual tastes, outperforming baselines while maintaining computational efficiency.

==> code/ncf.tex <==

class NCFModel(nn.Module):
    """Neural Collaborative Filtering Model"""
    def __init__(self, num_users, emb_dim, d, mlp_layers=[128, 64, 32], dropout=0.2):
        super(NCFModel, self).__init__()
        self.num_users = num_users
        self.emb_dim = emb_dim
        self.d = d
        
        # GMF (Generalized Matrix Factorization) components - similar to original IRT
        self.user_embedding_gmf = nn.Embedding(num_users, d)
        self.user_bias = nn.Embedding(num_users, 1)
        self.item_transform_gmf = nn.Linear(emb_dim, d)
        self.item_bias = nn.Linear(emb_dim, 1)
        
        # MLP components for capturing nonlinear interactions
        self.user_embedding_mlp = nn.Embedding(num_users, d)
        self.item_transform_mlp = nn.Linear(emb_dim, d)
        
        # MLP layers
        mlp_input_dim = d * 2  # concatenated user and item embeddings
        self.mlp_layers = nn.ModuleList()
        prev_dim = mlp_input_dim
        
        for layer_dim in mlp_layers:
            self.mlp_layers.append(nn.Linear(prev_dim, layer_dim))
            self.mlp_layers.append(nn.ReLU())
            self.mlp_layers.append(nn.Dropout(dropout))
            prev_dim = layer_dim
        
        # Final fusion layer
        self.final_layer = nn.Linear(d + mlp_layers[-1], 1)
        
    def forward(self, U, E):
        # GMF component (linear interactions like original IRT)
        user_emb_gmf = self.user_embedding_gmf(U)  # [batch, d]
        item_emb_gmf = self.item_transform_gmf(E)  # [batch, d]
        gmf_output = user_emb_gmf * item_emb_gmf  # Element-wise product [batch, d]
        
        # MLP component (nonlinear interactions)
        user_emb_mlp = self.user_embedding_mlp(U)  # [batch, d]
        item_emb_mlp = self.item_transform_mlp(E)  # [batch, d]
        mlp_input = torch.cat([user_emb_mlp, item_emb_mlp], dim=1)  # [batch, 2*d]
        
        mlp_output = mlp_input
        for layer in self.mlp_layers:
            mlp_output = layer(mlp_output)
        
        # Combine GMF and MLP outputs
        combined = torch.cat([gmf_output, mlp_output], dim=1)
        
        # Add biases (similar to original IRT)
        user_bias = self.user_bias(U).squeeze()  # [batch]
        item_bias = self.item_bias(E).squeeze()  # [batch]
        
        # Final prediction
        prediction = self.final_layer(combined).squeeze() + user_bias + item_bias
        return sigmoid(prediction)
